Grasping in Uncertain Environments: A Case Study For Industrial Robotic Recycling

Autonomous robotic grasping of uncertain objects in uncertain environments is an impactful open challenge for the industries of the future. One such industry is the recycling of Waste Electrical and Electronic Equipment (WEEE) materials, in which electric devices are disassembled and readied for the recovery of raw materials. Since devices may contain hazardous materials and their disassembly involves heavy manual labor, robotic disassembly is a promising venue. However, since devices may be damaged, dirty and unidentified, robotic disassembly is challenging since object models are unavailable or cannot be relied upon. This case study explores grasping strategies for industrial robotic disassembly of WEEE devices with uncertain vision data. We propose three grippers and appropriate tactile strategies for force-based manipulation that improves grasping robustness. For each proposed gripper, we develop corresponding strategies that can perform effectively in different grasping tasks and leverage the grippers design and unique strengths. Through experiments conducted in lab and factory settings for four different WEEE devices, we demonstrate how object uncertainty may be overcome by tactile sensing and compliant techniques, significantly increasing grasping success rates.

==> authors.tex <==
\author{\IEEEauthorblockN{Annalena Daniels}
\IEEEauthorblockA{\textit{Automatic Control Engineering} \\
\textit{Techn. University of Munich}, Germany\\
% Munich, Germany \\
a.daniels@tum.de}
\and
\IEEEauthorblockN{Sebastian Kerz}
\IEEEauthorblockA{\textit{Automatic Control Engineering} \\
\textit{Techn. University of Munich}, Germany\\
% Munich, Germany \\
sebastian.kerz@tum.de}
\and
\IEEEauthorblockN{Salman Bari}
\IEEEauthorblockA{\textit{Automatic Control Engineering} \\
\textit{Techn. University of Munich}, Germany\\
% Munich, Germany \\
s.bari@tum.de}
\and
\IEEEauthorblockN{Volker Gabler}
\IEEEauthorblockA{\textit{Automatic Control Engineering} \\
\textit{Techn. University of Munich}, Germany\\% Munich, Germany \\
v.gabler@tum.de}
\and
\IEEEauthorblockN{Dirk Wollherr}
\IEEEauthorblockA{\textit{Automatic Control Engineering} \\
\textit{Techn. University of Munich}, Germany\\
% Munich, Germany \\
dw@tum.de}
% \and
% \IEEEauthorblockN{Marion Leibold}
% \IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
% \textit{name of organization (of Aff.)}\\
% City, Country \\
% email address or ORCID}
}
